Human-Like Decision Making: Document-level Aspect Sentiment Classification via Hierarchical Reinforcement Learning

Recently, neural networks have shown promising results on Document-level Aspect Sentiment Classification (DASC). However, these approaches often offer little transparency w.r.t. their inner working mechanisms and lack interpretability. In this paper, to simulating the steps of analyzing aspect sentiment in a document by human beings, we propose a new Hierarchical Reinforcement Learning (HRL) approach to DASC. This approach incorporates clause selection and word selection strategies to tackle the data noise problem in the task of DASC. First, a high-level policy is proposed to select aspect-relevant clauses and discard noisy clauses. Then, a low-level policy is proposed to select sentiment-relevant words and discard noisy words inside the selected clauses. Finally, a sentiment rating predictor is designed to provide reward signals to guide both clause and word selection. Experimental results demonstrate the impressive effectiveness of the proposed approach to DASC over the state-of-the-art baselines.

==> content/data_annotation.tex <==
\section{Data Collection and Annotation}
We collect 150k QA style reviews from \emph{Taobao}\footnote{http://www.taobao.com}, the most famous electronic business platform in China. The QA style reviews consists of three different domains: \emph{Bags}, \emph{Cosmetics} and \emph{Electronics}. Owing to annotation is expensive and labor-consuming, we randomly select 10k QA text pairs from each domain to perform annotation. Specifically,
inspired by \cite{DBLP:conf/semeval/PontikiGPPAM14}, we define the aspect at two levels of granularity, i.e., aspect term and aspect category. Moreover, like \cite{DBLP:conf/semeval/PontikiGPMA15}, we define three sentiment polarities, i.e., \emph{positive}, \emph{negative} and \emph{neutral} (mildly positive or mildly negative) towards both aspect terms and categories. Then, each QA text pair is annotated as two tuples (\emph{aspect term}, \emph{polarity}), (\emph{aspect category}, \emph{polarity}). More concretely, the annotation process mainly contains two stages:

\textbf{Stage 1: Aspects Terms and Polarities.} We annotate the single/multi-word terms together with its polarities inside each QA text pair according to three main guidelines:

\noindent \textbf{(1)} We only annotate the aspect terms when the question and answer are matched. For example, the QA text pair in Figure \ref{fig:one-example} is annotated as (``\emph{battery life}'', \emph{positive}) and (``\emph{operating speed}'', \emph{negative}) due to words ``\emph{durable}'', ``\emph{slow}'' and ``\emph{obtuse}''. However, in \textbf{E1}, the answer does not reply to the question correctly and thus ``\emph{ios}'', ``\emph{screen}'' and ``\emph{windows os}'' should not be annotated. 
\begin{enumerate}
\item[\textbf{E1:}] Q: \emph{How is ios of this laptop? How about the screen?}\\
A: \emph{Windows os is good.}
\end{enumerate}

% \noindent \textbf{(2)} The annotators should annotate the maximal noun phrase (the entire conjunction or disjunction) as a single aspect term. 
\noindent \textbf{(2)} We only annotate the aspect term towards which an opinion is expressed. For example, \textbf{E2} conveys only objective information without expressing opinions and thus ``\emph{laptop}'' should not be annotated.
\begin{enumerate}
\item[\textbf{E2:}] Q: \emph{How about this laptop?}\\
A: \emph{I bought this laptop yesterday.}
\end{enumerate}

\noindent \textbf{(3)} We only annotate aspect terms which explicitly name particular aspects. For example, in \textbf{E3}, ``\emph{this}'', ``\emph{it}'' should not be annotated.
\begin{enumerate}
\item[\textbf{E3:}] Q: \emph{Is this expensive? Did anybody buy one?}\\
A: \emph{Of course, it's quite expensive.}
\end{enumerate}


\begin{table}[t]
\centering
\vspace{1ex}

  \begin{tabularx}{\linewidth}{>{\small} p{1.5cm} >{\small} X}

%   \centering
  \toprule
  \textbf{Domains} & \multicolumn{1}{>{\small}c}{{Aspect Categories}}\\ 
   
  \hline
\multirow{3}{*}{\emph{Bags}} & {\emph{Size, Price, Appearance, Quality, Weight, Certified Products, Smell, Accessories, Material, Life Timer, Style, Workmanship, Color, Stain Resistant, Practicality}}   \\ 
  \hline
\multirow{4}{*}{\emph{Cosmetics}}  & \emph{Price, Efficacy, Moisturizing Performance, Certified Products, Adverse Reaction, Exfoliator, Texture, Long Lasting, Smell, Material, Noticeable Color, Quality, Colour, Touch, Skin Whitening, Acne}   \\
  \hline
\multirow{4}{*}{\emph{Electronics}} & \emph{System Performance, Appearance, Battery, Computing (e.g., cpu, gpu, tpu etc.), Certified Products, Quality, IO (e.g., keybord, screen, etc.), Price, Storage, Function (e.g., touch id, waterproof etc.)} \\ 

  \toprule
%   \end{tabularx}
\end{tabularx}
  \setlength{\belowcaptionskip}{-2 ex}
  \captionsetup{font={small}} 
\caption{List of defined aspect categories in each domain}
    \label{tab:datasets-aspect} 
\end{table}


\textbf{Stage 2: Aspects Categories and Polarities.} As shown in Table \ref{tab:datasets-aspect}, we first define 15, 16, 10 aspect categories for \emph{Bags}, \emph{Cosmetics} and \emph{Electronics} respectively. Then, we annotate aspect categories (chosen from these predefined category inventories) discussed in each QA text pair according to similar guidelines in Stage 1. For example, there are two aspect categories discussed in Figure \ref{fig:one-example}, i.e., category \emph{Battery} and \emph{System Performance}. Thus, the QA text pair is annotated as (\emph{Battery}, \emph{positive}) and (\emph{System Performance}, \emph{negative}).  After finished {Stage 1 and 2}, we discard the QA text pairs which have no annotated term and category.

We assign two annotators to annotate each QA text pair, and \textit{Kappa} consistency check value of the annotation is 0.81. When annotators cannot reach an agreement, an expert will make the final decision, ensuring the quality of data annotation. Table \ref{tab:datasets} shows statistics of the final annotated corpus. 
In addition, to motivate other scholars to investigate this new task,  we share the data together with detail annotation guidelines via github\footnote{Dataset URL is omitted due to review reason.}. 


\begin{table}[t]
\centering
\vspace{1ex}
  \begin{tabular}{>{\small}l>{\small}c>{\small}>{\small}c>{\small}c>{\small}c>{\small}c}
  \toprule
  \textbf{Domains} & \emph{Pos.} & \emph{Neg.} & \emph{Neu.}  &\emph{All} & \emph{\#Term}\\ 
  
  \hline
\emph{Bags} & 3003 & 724 & 153 & 3880 & 451 \\ 
\emph{Cosmetics}  & 3134 & 956 & 203 & 4293 & 621 \\ 
\emph{Electronics} & 2942 & 720 & 237 & 3899 & 343 \\ 

  \toprule
  \end{tabular}
  \setlength{\belowcaptionskip}{-2 ex}
  \captionsetup{font={small}} 
  \caption{Sample distribution of three domains (\emph{Pos.}, \emph{Neg.} and \emph{Neu.} denote \emph{positive}, \emph{negative} and \emph{neutral}; \emph{\#Term} denotes the number of aspect term in each domain)}
  \label{tab:datasets} 
\end{table}




==> content/useless.tex <==
% second sentence ``\emph{However operating speed is quite slow and obtuse}'' in \textbf{A} actually does not match first sentence ``\emph{How is battery life?}'' in \textbf{Q}, but corresponds to second sentence ``\emph{How about the operating speed of this phone?}'' in \textbf{Q} owing to both of them explicitly mention aspect "operating speed". Moreover, although first sentence ``\emph{Good, very durable.}'' in \textbf{A} mentions no explicit aspect, we can still match it with the first sentence in \textbf{Q} due to implicit semantic matching information between them for aspect ``\emph{battery life}''. Therefore, a well-behaved approach should be capable of precisely capturing the semantic matching information between question and answer for a specific aspect.


% \setlength{\tabcolsep}{1.8pt}
% \begin{table*}[t]
% 	\renewcommand{\arraystretch}{1.2}
% 	\addtolength{\tabcolsep}{2pt}
% 	\begin{center}
% 		\begin{small}
% 			\begin{tabular}{l  cccc cccc cccc}
% 				    \toprule
% 					  		& \multicolumn{4}{c}{\emph{Bags}} & \multicolumn{4}{c}{\emph{Cosmetics}} & \multicolumn{4}{c}{\emph{Electronics}}  \\ 
% 							\cmidrule(lr){2-5}		\cmidrule(lr){6-9}	\cmidrule(lr){10-13}
% 					Approaches &P &R &F1 &Acc.
% 					        &P &R &F1 &Acc
% 					        &P &R &F1 &Acc.\\ 
% 					\hline
% 					\hline
% 					{RAM} (Chen et al., 2017)   
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
					
% 					{GCAE} (Xue et al., 2018)	
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
					
% 					{Clause-AN}	(Wang et al., 2018a)
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
					
% 					{SA-LSTM}(Wang et al., 2018b)
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
					
% 					{HMN}	(Shen et al., 2018a)		
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
					
% 					\hline
% 					\hline
					
% 					{HAN-Soft}                  		
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\

% 					{HRAN w/o seg}  	
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
					
% 					{HRAN w/o RSN} 
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
					
% 					{HRAN w/o RBAN} 
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
					
% 					{HRAN}			             
% 					& 83.1 & 83.0 & 83.1 & 64.3   
% 					& 72.9 & 71.4 & 72.1 & 44.8  
% 					& 81.6 & 76.5 & 51.5 & 85.1 \\
% 					\bottomrule
% 			\end{tabular}
% 				\caption{Results of all approaches on QA aspect \textbf{category-level} sentiment classification in all domains. } 
% 			\label{table:conll05-all}
% 		\end{small}
% 	\end{center}
% \end{table*} 



% \textbf{(2)} Second, we annotate aspect  category (from predefined category set) in which the previous each annotated aspect term fall. For example, there are two aspect categories discussed in Figure \ref{fig:one-example}, i.e., category \emph{battery} and \emph{performance} which are corresponding to term ``\emph{battery life}'' and ``\emph{operating speed}'' respectively. 

% \textbf{(1) Baselines.}

% We employ some existing ASC approaches to QA-ASC as baselines. Note that, the input of all these approaches should be a single sequence and thus we concatenate question and answer text so as to generate a single sequence. Besides, we also implement several text matching approaches as baselines. 

% which captures importance of contexts for a aspect with a deep memory network.
% \noindent $\bullet$ \textbf{IAN:} This approach is an interactive learning approach, which can model contexts and aspects interactively. This is another state-of-the-art approach proposed by Ma et al., 2017.

% \noindent $\bullet$ \textbf{HN.} This is a basic hierarchical framework approach with sentence segmentation but without considering aspect information, i.e., removing $v_a$, $m_i$ in Eq.(6) and $v_a$, $M_{ij}$ in Eq.(10). This approach is similar to the approach proposed by \newcite{DBLP:conf/emnlp/ShenSWKLLSZZ18}.

% \noindent $\bullet$ \textbf{HAN-Soft.} This is a soft-attention based hierarchical framework approach, i.e., removing $m_i$ and $M_{ij}$ in Eq.(6) and Eq.(10) in order to substitute RASAM in both RBAN and RSN with soft-attention mechanism.


% \noindent $\bullet\ $\textbf{HRAN w/o RSN.} This is one version of our approach without RSN.
% , i.e., removing Eq.(16)-(19) and encoding the outputs of RBAN through a standard LSTM layer followed by the \emph{softmax} layer.

% \noindent $\bullet$ \textbf{HRAN w/o RBAN.} This is one version of our approach without RBAN.
% % , i.e., removing $v_a$ and $M_{ij}$ in Eq.(12).

% \textbf{(2) Our approaches:} Besides, in order to see how well the RAWS and RASAM work, we implement several versions of our approach. All above approaches employ same \textbf{Word Representation}.

% \noindent $\bullet\ $\textbf{RAWS.} This is one version of our approach without employing sentence segmentation. Like above baselines, we concatenate question and answer text to generate a sequence and then employ RASAM over this sequence.

% \noindent $\bullet$ \textbf{RAM.} This is a state-of-the-art deep memory network approach proposed by \newcite{DBLP:conf/emnlp/ChenSBY17}.


% Then, inspired by Shen et al., 2018, the objective of learning $\theta_r$ in RBAN is to maximize the expected reward, i.e.,
% \begin{equation}
% \begin{split}
% J(\theta_r)=\mathbb{E}_{(\mathcal{P},\pmb{x_{aspect}},y) \sim \mathcal{D}}\{\mathbb{E}_{\pmb{\hat{o}} \sim \hat{p}_\pi}[\mathcal{R}']\}\\
% \approx \frac{1}{N} \sum_i ^N \mathbb{E}_{\pmb{\hat{o}}\sim \hat{p}_\pi}[\mathcal{R}']\ \ \ \ \ \ \ \ \ \ \hspace{4ex}
% \end{split}
% \end{equation}
% where $N$ is the number of training samples, $\pmb{\hat{o}} =(\pmb{o^q},\pmb{o^a}) \sim\hat{p}_\pi(\pmb{\hat{o}}|\cdot;\theta_r)=p_\pi^q(\pmb{o^q}|\cdot)*p_\pi^a(\pmb{o^a}|\cdot)$. 


% \textbf{Step 1: Aspects terms and polarities} we annotate aspect terms inside each QA text pair, such as ``\emph{battery life}'' and ``\emph{operating speed}'' in Figure \ref{fig:one-example}. Meanwhile, we annotate the aspect categories (chosen from predefined category inventories) discussed in each QA text pair. For example, there are two aspect categories discussed in Figure \ref{fig:one-example}, i.e., category \emph{battery} and \emph{performance}. 
% Note that, like \newcite{DBLP:conf/semeval/PontikiGPMA15}, we only annotate the aspect term/category towards which an opinion is expressed. 

% \textbf{(2) BERT:} Devlin et al., 2018 recently propose to produce deep word representations with bidirectional encoder representations from transformers (BERT), and show that simply using the learned external word representations as extra inputs can effectively boost performance of a variety of tasks, including sentiment classification. Thus, in this study, we concatenate our learned word vector with extra BERT word vector as the final word representation of HRAN.

% \textbf{Sentence Segmentation:} We adopt Stanford CoreNLP (Manning et al.,
% 2014)\footnote{https://stanfordnlp.github.io/CoreNLP/ssplit.html} to segment all QA text pairs into sentences.

% \textbf{Sentence Segmentation.} We adopt Stanford CoreNLP \cite{DBLP:conf/acl/ManningSBFBM14} to segment all QA text pairs into sentences.



% However, our approach \textbf{RASA} outperforms all four state-of-the-art baselines, which highlights the importance of employing reinforced aspect-specific attention mechanism (RASAM) to replace soft-attention mechanism for QA-ASC task. Besides, when we empoly sentence segmentation, our approach \textbf{HN} without considering aspect information achieves comparable or even better performance than some state-of-the-art baselines, which confirms the helpfulness of of employing hierarchical framework to QA-ASC. 


% (1) The first term is a future cumulative reward $r^l(u_i)$ defined by Eq.(6) which is the final reward received by low-level policy after the selection of all words in $i$-th selected EDU are finished. Note that, if the $i$-th EDU is discarded, $r^l=0$. (2) The second rew
 
%  Second, since we aim to select aspect-relevant EDUs, we define an aspect-relevant intermediate reward based on $cosine$ similarity between aspect representation $v_a \in \mathbb{R}^d$ and hidden state $\hat{v}_i \in \mathbb{R}^d$ of the $i$-th EDU $u_i$.

% $\gamma$ is a discount factor; 
% Third, after $\LSTM_{\pi}^h$ finishes all options, we feed the last hidden state $\hat{v}_n$ to rating predictor. Then we regard the loss of classifier, i.e., $\log p(y|({T},{x_{aspect}})$ in Eq.(8) as another delay reward


%  $\bullet$ \textbf{LSTM.} This approach only adopts a stantard LSTM network to model the text without considering aspect information \cite{DBLP:conf/emnlp/WangHZZ16}.
%  $\bullet$ \textbf{W\&C-AN.} This is another state-of-the-art approach with  both word and clause-level attention  proposed by \cite{DBLP:conf/ijcai/WangLLKZSZ18}.

%  $\bullet$ \textbf{DAN.} This is a deep averaging fully connected network with averaged word embeddings as input \cite{DBLP:conf/emnlp/YinSZ17}.
